ReadOnce Transformers: Reusable Representations of Text for Transformers

We present ReadOnce Transformers, an approach to convert a transformer-based model into one that can build an information-capturing, task-independent, and compressed representation of text. The resulting representation is reusable across different examples and tasks, thereby requiring a document shared across many examples or tasks to only be \emph{read once}. This leads to faster training and evaluation of models. Additionally, we extend standard text-to-text transformer models to Representation+Text-to-text models, and evaluate on multiple downstream tasks: multi-hop QA, abstractive QA, and long-document summarization. Our one-time computed representation results in a 2x-5x speedup compared to standard text-to-text models, while the compression also allows existing language models to handle longer documents without the need for designing new pre-trained models.

==> images/repr_tablev1.tex <==

\begin{table}[ht]
    \centering
    \footnotesize
    \renewcommand{\tabcolsep}{0.8mm}
    \begin{tabular}{l|ccc}
     \multirow{2}{*}{Architecture} & \hotpot & \nqa & \xsum \\
      & F1 & R-L & R-L \\
      \midrule
    %   \cmidrule{2-5}
    $\sysshortername_{\phi}$(Bart-L; K=8) & 64.8 & 41.9 & 32.6 \\
    \sysshortername(Bart-L; K=8) & 70.9 & 55.7 & 31.9 \\
    \sysshortername(Bart-L; K=2) & \textbf{77.2} & \textbf{66.7} & \textbf{35.4} \\
    \bart-L  & 80.2 & 69.3 & 37.3 \\
     BART-L$_\text{{\squad+\unsup}}$ & 80.1 & 70.5 & 37.2 \\
     \midrule
    \sysshortername(Bart-B; K=2) & 71.5 & 61.3 & 31.6 \\
    BART-B$_\text{{\squad+\unsup}}$ & 76.5 & 65.8 & 32.2 \\
    \midrule
    \sysshortername(DistilBART; K=2) & 75.5 & 65.1 & 33.4 \\
    % \multicolumn{4}{c}{Upper Bounds} \\
    % Upper Bounds &&& \\
    % \multirow{2}{*}{\rotatebox[origin=c]{90}{Upper \\ Bound}}& & & \\
    % \cmidrule{1-1}
     DistilBART$_\text{{\squad+\unsup}}$ & 80.5 & 70.5 & 36.5 \\
    \end{tabular}
    \caption{
        Performance of \sysname on three datasets, vs.\ a standard text-to-text transformer with full access to document text. Competitive performance at K=2 indicates our document representation is effective at capturing information.
    }
    \label{tab:repr}
\end{table}
